Memory Scraping Attack on Xilinx FPGAs: Private Data Extraction from Terminated Processes

FPGA-based hardware accelerators are becoming increasingly popular due to their versatility, customizability, energy efficiency, constant latency, and scalability. FPGAs can be tailored to specific algorithms, enabling efficient hardware implementations that effectively leverage algorithm parallelism. This can lead to significant performance improvements over CPUs and GPUs, particularly for highly parallel applications. For example, a recent study found that Stratix 10 FPGAs can achieve up to 90\% of the performance of a TitanX Pascal GPU while consuming less than 50\% of the power. This makes FPGAs an attractive choice for accelerating machine learning (ML) workloads. However, our research finds privacy and security vulnerabilities in existing Xilinx FPGA-based hardware acceleration solutions. These vulnerabilities arise from the lack of memory initialization and insufficient process isolation, which creates potential avenues for unauthorized access to private data used by processes. To illustrate this issue, we conducted experiments using a Xilinx ZCU104 board running the PetaLinux tool from Xilinx. We found that PetaLinux does not effectively clear memory locations associated with a terminated process, leaving them vulnerable to memory scraping attack (MSA). This paper makes two main contributions. The first contribution is an attack methodology of using the Xilinx debugger from a different user space. We find that we are able to access process IDs, virtual address spaces, and pagemaps of one user from a different user space because of lack of adequate process isolation. The second contribution is a methodology for characterizing terminated processes and accessing their private data. We illustrate this on Xilinx ML application library.

==> Futurework.tex <==
Our current research primarily centers on the Xilinx ZCU104 platform, but we intend to broaden our scope to include Intel's FPGAs and other high-end FPGAs commonly used in cloud environments in the future. It's essential to clarify that the attacks and solutions presented here are specific to Zynq Ultrascale+ MPSoC architectures running PetaLinux with the Xen hypervisor variant. Additionally, our objective is to develop a practical solution for initializing data from previous guest users in various virtualization environments.

==> Rebuttal.tex <==
We would like to thank all the reviewers for their time and constructive criticism on the paper. 

Common Concerns: 

Scientific Contributions and Novelty: While many FPGAs prioritize safeguarding active processes, they frequently overlook the essential task of clearing memory contents for terminated processes, with potentially severe consequences. The significance of this issue arises from the failure to recognize the potential fallout of neglecting to initialize the memory area of a concluded process. Notably, NVIDIA's lack of comprehension resulted in them not addressing this issue. Attackers capitalized on this vulnerability, employing a similar method to access residual data in the DRAM left behind by a GPU-driven process. Their success included image reconstruction and sensitive data retrieval from these terminated processes. Our investigation of this hypothesis subsequently confirmed that memory contents of terminated processes remain intact in the ZCU104 FPGA environment, with potential catastrophic ramifications – marking our primary contribution. 

Embedded systems operate within resource-constrained environments, where embedded operating systems like PetaLinux, Xilinx's proprietary system, oversee memory isolation akin to other embedded OSs. However, due to FPGA board constraints, PetaLinux lacks the extensive features found in traditional OSs within standard System on Chips (SoCs). Moreover, FPGAs prioritize accelerated processing, leading to trade-offs between software and hardware checks. This often involves reducing runtime checks to optimize execution speed and efficiency. Despite these limitations, PetaLinux does not clear memory locations of terminated processes, inadvertently granting unprivileged users access to critical information stored in memory. Basic users may be unaware of clearing memory locations or the intricacies of physical memory addresses and page table conversions, leaving them ignorant of potential memory attacks after termination – signifying our second contribution.

Our third contribution emphasizes the feasibility of such attacks, especially relevant in multi-tenant scenarios utilizing local FPGA memory. Adversarial tenants can exploit PetaLinux's unrestricted access, gaining sensitive details about other tenants or processes. This vulnerability allows them to retrieve data from onboard memory even after a tenant's termination. Clearing memory after a process is terminated is paramount in multi-tenant scenarios to ensure data privacy, maintain isolation, enhance security, adhere to regulations, build trust, and prevent information leakage. Implementing proper memory management practices is essential to maintain the integrity and security of shared hardware resources.

Each manufacturer employs its own empirical methods to enhance process execution speed, often overlooking the security implications associated with terminated processes. Implementing a comprehensive operating system solution isn't feasible due to resource constraints on the onboard capacities.

While our contributions might not be groundbreaking in terms of their novelty, they do embody a straightforward and effective approach. This illustrates that even a relatively simple attack, like the one we've demonstrated, can successfully reveal the memory contents of a terminated process. This serves as a powerful reminder that the vulnerability we've identified is not confined to complex methods but can be exploited using basic techniques.

Questions:
Reviewer 3: 
1) "Zynqs and Peta Linux actually used in datacenters?.. "
Yes they are used in data centers. A web search showed Google, Facebook , Cisco using Zynq operated by Petalinux for a variety of tasks.The users run their applications as processes on the FPGA.
2) "I suppose only one user ever has possession of an FPGA acceleration board and is running their process there until it is restarted?"
 No. In a multi-tenant scenario, numerous users can access distinct resources on the board, managed and scheduled by PetaLinux without the FPGA being restarted.
3) "Implementations need to take care of zeroization." 
Not all users are familiar with page tables or a means to identify the location of their data in FPGA memory for content clearing. Additionally, the FPGA lacks feature capability for users to zero their memory locations before termination. 

Reviewer 4: 
1) Step2, 3 require root privileges? 
In the event that the adversary is an AMD system debugger, which is designed for legitimate use and operates without requiring root privileges, they can potentially exploit this debugger to profile sensitive information and execute a memory attack. If permitted, we will provide a comprehensive explanation of this scenario.
2) "Assuming step 3 does not require root privileges (as stated by the authors in Section 3), then the adversary could anyways read out the whole DRAM content. "?
Indeed, it's possible to read out the entire DRAM, but the time needed for such an operation would be extensive. This is precisely why we opt for a targeted attack, capitalizing on vulnerabilities in PetaLinux to achieve our objectives efficiently. 
3) "FPGAs are never "equipped with CPUs" ... FPGAs cannot "execute applications" (L114) ... "?
As per AMD's technical reference, the Zynq ZCU104 FPGA includes A53 ARM processors (APUs) emulating CPU functions within a limited SoC capacity. The board's DPUs and RPUs are dedicated to running machine learning applications, such as the resnet50 model executed on the DPU of the AMD-provided ZCU104 board.

In the event that our paper is accepted or we are granted an opportunity to resubmit with revisions, we are committed to addressing the specific concerns raised by reviewers 3 and 4, as well as addressing  other concerns that are not explicitly mentioned above.

==> codeavailability.tex <==
Code will be made available at GitHub at the time of the publication of this paper.

